Hierarchical reinforcement learning for efficient exploration and transfer

Sparse-reward domains are challenging for reinforcement learning algorithms since significant exploration is needed before encountering reward for the first time. Hierarchical reinforcement learning can facilitate exploration by reducing the number of decisions necessary before obtaining a reward. In this paper, we present a novel hierarchical reinforcement learning framework based on the compression of an invariant state space that is common to a range of tasks. The algorithm introduces subtasks which consist of moving between the state partitions induced by the compression. Results indicate that the algorithm can successfully solve complex sparse-reward domains, and transfer knowledge to solve new, previously unseen tasks more quickly.

==> algo.tex <==

\usepackage{algorithmic}
\usepackage{algorithm}
\begin{document}
\begin{algorithm}
\caption{\textsc{HRL}}
\begin{algorithmic}[1]
		 \STATE {\bf Input}: MDP $\mathcal{M}$, initial state $s_0\in S$
		 \STATE $s\gets s_0$: current state
		 \STATE $v$: graph node storing the initial region $f(s_0)$
		 \STATE $G\gets (\{v\},\emptyset)$ // graph containing graph node $v$ and no edges
		 \WHILE{within budget}
			  \STATE $v' \gets $ \textsc{SelectNeighbor}($v$)
			  \STATE $o \gets $ \textsc{GetOption}($v,v'$)
    		   \STATE $s \gets $ \textsc{RunOption}($o, v'$)
    		   \STATE $v'\gets $ \textsc{GetNodeWithRegion}($G, f(s)$) // create node if needed
			   \IF{$(v,v')\notin E$}
    				\STATE append edge $(v,v')$ to $HRLE$
    				\STATE create option $o_{v,v'}$ for performing the transition from $v$ to $v'$
			   \ENDIF
	  \ENDWHILE
 \end{algorithmic}
 \label{algo: hrl}
\end{algorithm}

\begin{algorithm}
	\caption{\textsc{RunOption}}
	\begin{algorithmic}[1]
				  \WHILE{$f(s) = z(v)$}
					   \STATE $a \gets$ \textsc{SelectAction}($o$)
					   \STATE $s \sim P(\cdot | s,a)$
				  \ENDWHILE
				  \IF {$f(s)=v'$}
					   \STATE reward option $o$
				   \ELSE
					   \STATE punish option $o$
					 \ENDIF
	 \end{algorithmic}
	 \label{algo: run_option}
\end{algorithm}

\begin{algorithm}
	\caption{\textsc{GetOption}}
	\begin{algorithmic}[1]
		 \STATE {\bf Input}: G $\mathcal{G}$, initial state $s\in S$
		 \STATE $o = arg\max_{o \in E} Q(f(s),o)$
	 \end{algorithmic}
	 \label{algo: get_option}
\end{algorithm}

\begin{algorithm}
	\caption{\textsc{Update Manager}}
	\begin{algorithmic}[1]
		\STATE {\bf Input}: $(z, o, r, z')$
		\STATE $Q(z, o) \gets Q(z,o) + \alpha \left[r + \gamma \max_{o'} Q(z', o') - Q(z, o) \right]$
	 \end{algorithmic}
	 \label{algo: hrl}
\end{algorithm}

\begin{algorithm}
	\caption{\textsc{Update Options}}
	\begin{algorithmic}[1]
		\STATE {\bf Input}: $(s, a, r, s')$
		\STATE $L(\eta_\theta)(s,a,r,s')$
		\STATE $L(\hat{V}_\psi)(s,a,r,s')$
	 \end{algorithmic}
	 \label{algo: hrl}
\end{algorithm}
\end{document}{}

